Prompt-Based Metric Learning for Few-Shot NER

Few-shot named entity recognition (NER) targets generalizing to unseen labels and/or domains with few labeled examples. Existing metric learning methods compute token-level similarities between query and support sets, but are not able to fully incorporate label semantics into modeling. To address this issue, we propose a simple method to largely improve metric learning for NER: 1) multiple prompt schemas are designed to enhance label semantics; 2) we propose a novel architecture to effectively combine multiple prompt-based representations. Empirically, our method achieves new state-of-the-art (SOTA) results under 16 of the 18 considered settings, substantially outperforming the previous SOTA by an average of 8.84% and a maximum of 34.51% in relative gains of micro F1. Our code is available at https://github.com/AChen-qaq/ProML.

==> limitation.tex <==
\section{Limitations}
Although our \ours achieves substantially improvements for few-shot NER tasks, it is still not good enough compared with standard full-label supervised NER results. Note that the performance on the GUM dataset is quite poor, suggesting that in the domain transfer setting, the gap between source domain and target domain will largely affect the performance.
It still remains a critical challenge to close the gap between full-label models and few-shot models in the setting of few-shot NER.
% Therefore, it is still not applicable for high-stake employments, and more researches need to be done in future.
